The Shapley Value in Machine Learning

Over the last few years, the Shapley value, a solution concept from cooperative game theory, has found numerous applications in machine learning. In this paper, we first discuss fundamental concepts of cooperative game theory and axiomatic properties of the Shapley value. Then we give an overview of the most important applications of the Shapley value in machine learning: feature selection, explainability, multi-agent reinforcement learning, ensemble pruning, and data valuation. We examine the most crucial limitations of the Shapley value and point out directions for future research.

==> sections/owen.tex <==
\subsection{The Owen value}
The Owen value is a generalization of the Shapley value concept to a setting where the coalition structure is constrained. Because such scenarios are relevant to machine learning applications we give an introductory level overview.
\begin{definition}
\textbf{Coalition structure.} A \textit{coalition structure} is a partition of $\mathcal{N}$. That is, $\mathcal{C} = \{\mathcal{C}_1, \dots, \mathcal{C}_m \}$ is a coalition structure if given $\mathcal{M}=\{1, \dots, m\}$ and $i \neq j$ it satisfies that $\bigcup_{i \in \mathcal{M}} \mathcal{C}_i = \mathcal{N}$ and $\mathcal{C}_i \cap \mathcal{C}_j = \emptyset$.
\end{definition}
\begin{definition} \textbf{Admissible permutation.} The permutation  $\pi \in \Pi( \mathcal{N})$ is admissible with respect to $\mathcal{C}$ if for any $i,j,k \in \mathcal{N}; i,k\in \mathcal{C}_l; \mathcal{C}_l \in \mathcal{C}$ the relation $\pi(i)<\pi(j)< \pi(k)$ implies that $j \in \mathcal{C}_l$. 
\end{definition}

Let us assume in our illustrative example that the coalition structure $\mathcal{C}$ is defined by: $\left\{\left \{ 1,3\right \}, \left\{2\right\}\right\}$. The permutation $(3, 1, 2)$ is admissible, while $(1, 2, 3)$ is not admissible.
\begin{definition} \textbf{Set of admissible permutations.} We denote by $\widetilde{\Pi} (\mathcal{N},\mathcal{C})$ the set of admissible permutations defined on $\mathcal{N}$ and $\mathcal{C}$.
\end{definition}
\begin{definition}
\textbf{Owen value.} The Owen value \cite{owen1977values} is a solution concept for cooperative games with a given coalition structure. The $i^{th}$ component of the single solution vector satisfying this solution concept for any cooperative game and coalition structure $(\mathcal{N}, v,\mathcal{C})$ is given by Equation \ref{eq:owen}.
{\small
\begin{align}
    \phi^{Ow}_i=\frac{1}{|\widetilde{\Pi} (\mathcal{N},\mathcal{C})|}\sum\limits_{\pi \in \widetilde{\Pi} (\mathcal{N},\mathcal{C})}\underbrace{[v(\mathcal{P}^{\pi}_i \cup \left\{ i\right\})-v(\mathcal{P}^{\pi}_i)]}_{\textbf{Marginal contribution of the i$^{th}$ player.}}\label{eq:owen}
\end{align}}
\end{definition}
The Owen value of a player is the average marginal contribution of the player to the payoff of the predecessor set based on every admissible permutation of the player set conditioned on the coalition structure. We included the marginal contributions and Owen values in Table \ref{tab:owen} based on the admissible permutations.
\input{tables/owen_example}

==> tables/applications_old.tex <==


\begin{table*}[h!]
\centering
\caption{An application area, player/coalition/payoff definition, Shapley value approximation technique, and computation time (the player set is noted by $\mathcal{N}$) based comparison of research works. Specific applications of the Shapley value are grouped together and ordered chronologically in the table.\rey{The last column should be refer to ``Sampling size''} }
{\scriptsize
\begin{tabular}{ccccccc}
\hline
 \textbf{Application}& \textbf{Reference} & \textbf{Player} & \textbf{Coalition} & \textbf{Payoff} & \textbf{Approximation} &\textbf{Time}\\
 \hline
%Feature Selection & \cite{cohen} & Feature & Feature set & Model performance & Exact &$\mathcal{O}(|\mathcal{N}|!)$ \\
Feature Selection & \cite{cohen2007feature} & Feature & Feature set & Validation loss & MSA &$\mathcal{O}(C^{|\mathcal{N}|}_d)$ \\
% d is the size of significant interactions between features
Feature Selection &\cite{patel2021game} & Feature & Feature set & Validation loss & Monte Carlo sampling &$O(|\mathcal{N}|)$\\
Feature Selection & \cite{tripathi2020interpretable} & Feature & Feature set & Training loss & Monte Carlo sampling &$O(|\mathcal{N}|)$ \\
Feature Selection &\cite{sun2012feature} & Feature & Feature set & Mutual information (MI) & Exact & $O(|\mathcal{N}|!)$\\
Feature Selection &\cite{guha2021cga} & Feature & Feature set & PCC \& MI & Exact & $O(|\mathcal{N}|!)$\\
%PCC: Pearson Correlation Coefficient
Feature Selection & \cite{williamson2020efficient} & Feature & Feature set & Variable importance & \tiny{Analysis on asymptotic distribution} & $\Theta (n)$\\
% $n$ is the size of the training data set, AD: Asymptotic distribution
\hline
 Data Valuation  & \cite{jia2019towards} &  &  &  &  &\\
 Data Valuation  & \cite{ghorbani2019data} & Validation accuracy & Monte Carlo sampling & O( & & \\
 Data Valuation  & \cite{shim2021online} &  &  &  & & \\
 Data Valuation  & \cite{deutch} &  &  &  &  &\\
 Data valuation  &  \cite{kwon2021efficient}&  &  &  &  &\\
 Data valuation  & \cite{kwon2021beta} &  &  &  &  &\\
\hline
Federated learning & \cite{liu2021gtg} &  &  &  &  &\\
\hline
 Explainability (Graphical Model) & \cite{liu2020shapley} &  &  &  &  &\\
 Explainability (Graphical Model) & \cite{singal21a} &  &  &  &  &\\
 \hline
 Explainability (DL) & \cite{chen2018shapley} &  &  &  &  &\\
 Explainability (DL) & \cite{ancona2019explaining} &  &  &  &  &\\
 Explainability (DL) & \cite{ghorbani2020neuron} &  &  &  &  &\\
 Explainability (DL) & \cite{zhang2021interpreting} &  &  &  &  &\\
\hline
 Explainability   & \cite{lundberg2017unified} &  &  &  &  &\\
 Explainability   & \cite{sundararajan2020shapley} &  &  &  &  &\\
 Explainability   & \cite{sundararajan2020many} &  &  &  &  &\\
 Explainability   & \cite{heskes2020causal} &  &  &  & & \\
 Explainability   & \cite{frye2020asymmetric}&  &  &  & & \\
 Explainability   & \cite{frye2020shapley}&  &  &  & & \\
 Explainability   & \cite{wang2021shapley} & Causal graph vertex & Causal subgraph & Attribution & & \\
 Explainability   & \cite{subgraphx_icml21} &  Vertex& Vertex set & Attribution & Monte Carlo sampling &$O(|\mathcal{N}|)$ \\
 Explainability   &\cite{covert2021improving}& Feature & Feature set  & Attribution& Linear Regression& $\mathcal{O}(|\mathcal{N}|)$\\
% Explainability   & \cite{covert2021explaining} &  &  &  &  &\\
\hline
 Multi-agent RL&\cite{wang2021shaq}  &  Agents& Cooperating agents & Global reward & Monte Carlo sampling  & $\mathcal{O}(|\mathcal{N}|)$\\\
  Multi-agent RL& \cite{shapcredit}& Agents & Cooperating agents & Global reward & Monte Carlo sampling & $\mathcal{O}(|\mathcal{N}|)$\\
\hline
Model valuation &  \cite{rozemberczki2021shapley}& Binary classifier & Ensemble & Predictive performance &Voting game& $\mathcal{O}(|\mathcal{N}|^2)$ \\
 \hline
\end{tabular}
}
\end{table*}

==> tables/owen_example.tex <==
\begin{table}[h!]
\caption{The admissible permutations of the players according to the coalition structure, marginal contributions of the players in each admissible permutation and the Owen values.}\label{tab:owen}
\centering
{\footnotesize
\begin{tabular}{cccc}
            & \multicolumn{3}{c}{\textbf{Marginal Contribution} }\\ \hline
\specialcell{\textbf{Admissible} \\\textbf{Permutation}} & \textbf{Player 1}     & \textbf{Player 2}     & \textbf{Player 3}    \\ \hline
(1, 3, 2)   &       7       &       4       &       14      \\
(2, 1, 3)   &       7       &       11       &      7       \\
(2, 3, 1)  &        2      &        11      &       12      \\
(3, 1, 2)   &       7       &       4       &       14      \\ \hline
\textbf{ Owen value } &     23/4        &      30/4        &        47/4     \\ \hline
\end{tabular}}
\end{table}
